LamRA: Large Multimodal Model as Your Advanced Retrieval Assistant

With the rapid advancement of multimodal information retrieval, increasingly complex retrieval tasks have emerged. Existing methods predominately rely on task-specific fine-tuning of vision-language models, often those trained with image-text contrastive learning. In this paper, we explore the possibility of re-purposing generative Large Multimodal Models (LMMs) for retrieval. This approach enables unifying all retrieval tasks under the same formulation and, more importantly, allows for extrapolation towards unseen retrieval tasks without additional training. Our contributions can be summarised in the following aspects: (i) We introduce LamRA, a versatile framework designed to empower LMMs with sophisticated retrieval and reranking capabilities. (ii) For retrieval, we adopt a two-stage training strategy comprising language-only pre-training and multimodal instruction tuning to progressively enhance LMM's retrieval performance. (iii) For reranking, we employ joint training for both pointwise and listwise reranking, offering two distinct ways to further boost the retrieval performance. (iv) Extensive experimental results underscore the efficacy of our method in handling more than ten retrieval tasks, demonstrating robust performance in both supervised and zero-shot settings, including scenarios involving previously unseen retrieval tasks.

==> section/01-introduction-old.tex <==
\section{Introduction}

% retrieval的现状和问题
\noindent Recently, the field of multimodal information retrieval has been significantly advanced by the remarkable success of Vision-Language Models (VLMs) \jc{may need to check whether you have some misunderstanding and misusing about VLMs and LMMs. Generally, LMMs $>$ VLMs. do not limit LMMs to visual and text modalities.}. For instance, CLIP~\cite{radford2021learning} and ALIGN~\cite{jia2021scaling}, which are trained through contrastive learning~\cite{oord2018representation} on large-scale image-text pairs, have demonstrated surprisingly impressive generalizability on cross-modal retrieval. 
However, as the landscape of information retrieval evolves, more challenging tasks have emerged, 
including, composed image retrieval~\cite{liu2021image, liu2023zero}, long-text image retrieval~\cite{zhang2024long}, and image/question to multimodal document retrieval~\cite{yan2024echosight, chen2023can}. 
\weidi{maybe go with `specialising on these diverse tasks can be challenging or laborious.' then say, `would be interest to design versatile retrieval scheme.'}


% 大模型的潜力以及为什么要用大模型来解决 retrieval 这个task
\weidi{maybe this paragraph should discuss the effort of modern LMMs in unifying vision-language tasks, for example, OFA, demonstrating flexibility, blabla...}
\weidi{discuss why this paradigm becomes successful, 
(i) tremendous success of training LLMs on large corpus of human-generated content, prior of the physical world, better understanding of natural languages;
(ii) language is a natural interface between machine and human agent, that naturally enables interactions for various tasks....}
\weidi{In this paper, we aim to formulate various of retrieval problems under the umbrella of LMMs, which exploits .... what benefit ....}

Since dual-encoder networks like CLIP aim to enhance the alignment between the image and text, they encounter challenges when dealing with interleaved image-text inputs. Moreover, the text encoder of CLIP exhibits a limited understanding of complex text~\cite{hsieh2024sugarcrepe, singh2024learn}. Consequently, there is an urgent need to develop new paradigms to address the diverse retrieval tasks effectively. 

In parallel, with the rapid advancement of Large Language Models (LLMs), LLMs have demonstrated exceptional capabilities across a range of tasks~\cite{brown2020language, wang2023improving, dubey2024llama, yan2024visa}, including question answering and text embedding extraction. Building on this success, Large Multimodal Models (LMMs) integrate visual and textual modality by mapping the image space to the language space of LLMs through visual instruction tuning. Unlike CLIP, which uses contrastive learning to achieve enhanced global representations, visual instruction tuning allows for 
the learning of more detailed, region-level image features~\cite{yu2022coca}. \weidi{not sure the above claim is correct.} Moreover, LMMs inherently possess a deeper understanding of textual modality and can handle more flexible input formats. This raises a pertinent question: can LMMs establish a new paradigm for addressing diverse retrieval tasks? 

% 我们的方法
\weidi{Our goal is to ... with minimal training cost ? Specifically, we insert light-weight LoRA modules into .... that expands the ability of LMMs with retrieval, while maintaining .... without LoRAs inserted. At training time, we consider a two-stage training strategy ...}

\jc{it seems that we go from versatile LLM down to retrieval. This makes you lack of comprehensive discussion about the retrieval development. It is ok but suggest to add more literature citations in retrieval area.}

To answer the above question, this paper introduces \textbf{LamRA}, a comprehensive framework designed to equip LMM with advanced retrieval and reranking capabilities. Specifically, to enable LMM to perform effective retrieval, we propose a two-stage training strategy aimed at progressively refining their retrieval performance. 
The first stage is pre-training, in which we strengthen the LMM's ability to extract single-modal embeddings.
\weidi{unclear what do you mean by `extract single-modal embeddings'}
The second stage involves instruction tuning, where the model is fine-tuned using a diverse set of retrieval datasets. This step aims to further improve the model's adaptability to a range of retrieval tasks. To further equip LMMs with reranking capabilities and leverage their ability to process flexible inputs, we employ hard sample mining on the trained retrieval model, enabling joint training for both pointwise and listwise reranking. The resulting reranker model supports inputs of single or multiple candidates to further optimize overall retrieval performance.

To evaluate the effectiveness of our method across diverse retrieval tasks, we conduct experiments on more than ten distinct retrieval tasks. \weidi{for example, image-to-text, text-to-image, .....}
The results indicate that our method demonstrates robust performance on both in-domain and out-of-domain retrieval datasets. Additionally, we perform exploratory experiments on several Knowledge-based Visual Question Answering (KVQA) benchmarks. The experimental results show the feasibility of integrating retrieval and generative capabilities within a single LMM. \weidi{give a table on the benchmarks or tasks we have been doing.}

% 三个 contribution 
In a nutshell, our contributions are as follows:


==> section/03-method.tex <==
\section{Method}

This section starts by formulating our considered problem in Section~\ref{sec:problem_formulation}; then we elaborate on the architecture and feature extraction process in Section~\ref{sec:feature_extraction}; and describe the training details to equip the LMMs with retrieval capability in Section~\ref{sec:training_for_retrieval}; then, we present the approach to endow the LMMs with universal reranking abilities in Section~\ref{sec:reranking}, aiming to further boost retrieval performance; lastly, we detail the inference pipeline of our method in Section~\ref{sec:inference}.

\subsection{Problem Formulation} 
\label{sec:problem_formulation}

We address the challenge of universal retrieval and reranking with a generative model. Specifically, for one specific query~($q$), which can be an image, text, or an interleaved image-text format, and a retrieval set of $N$ candidates $\Omega = \{c_1, c_2, \cdots, c_N\}$ where each $c_i$ comprises images, text, or interleaved formats, we first extract the embeddings for both the query and all candidates with LMMs, and rank all candidates in $\Omega$ based on the relevance, 
{\em i.e.}, cosine similarity between the query and candidate embeddings. 
This initial retrieval process yields the top-$K$ candidates, represented as $\mathcal{C}_1 = \Phi_{\text{ret}}(q, \Omega)$. Subsequently, we refine this subset through a reranking process to produce the final ranked output, denoted as $\mathcal{C}_2 = \Phi_{\text{rerank}}(q, \mathcal{C}_1)$. Here, $\mathcal{C}_2$ represents the final reordered set of candidates.

In the following section, we provide details on extracting features for queries and candidates of arbitrary format.

% \weidi{need to provide more details, 
% how images and texts are encoded, and get the embedding, 
% then what is the task, i.e., rank the cases in a pool by relevance score, .... 
% what does reranking looks like,....}
% \weidi{need to provide a formulation for this universal retrieval problem, for example, assume a set of images $\mathcal{I} = \{I_1, I_2, \dots, I_n\}$, ...}

\subsection{Architecture \& Feature Extraction}
\label{sec:feature_extraction}

Generally speaking, the architecture of Large Multimodal Models~(LMMs) typically consists of three main components: a vision encoder, a vision projector, and a language model. To compute the embedding with a generative model, 
we adopt a similar approach as ~\cite{jiang2023scaling, jiang2024e5},
using an Explicit One-word Limitation (EOL). 
Specifically, we use the following prompts: 
(i) for image-only input, we use: \texttt{<image> Summarize above image in one word: <emb>}; 
(ii) for text-only input, we use: \texttt{<text> Summarize above sentence in one word: <emb>};
(iii) for mixed image-text input, we utilize: \texttt{<image\textsubscript{1}><text\textsubscript{1}>...<image\textsubscript{i}><text\textsubscript{j}> Summarize above image and sentence in one word: <emb>.} 
where \texttt{<image>} and \texttt{<text>} denote placeholders for the input image and sentence, respectively. For any combination of images and text inputs, the LMM uses the vision encoder and vision projector to map images into language space, which are then processed alongside the text by the large language model. 
We use the last hidden state immediately preceding the \texttt{<emb>} token as the representation of the input.

\subsection{Training for Retrieval} 
\label{sec:training_for_retrieval}

\vspace{2pt}\noindent 
In this section, we describe a two-stage training scheme, to advance the retrieval capabilities of LMMs. The first stage involves language-only pre-training, which facilitates the generative model to output improved embeddings. 
The second stage, instruction tuning, further adapts the LMMs to a wide range of retrieval tasks.

\vspace{2pt}
\noindent \textbf{Stage-I: Adapting LMMs for Retrieval Tasks.} 
LMMs were trained for generative tasks, {\em e.g.}, next-token prediction, which limits their ability for retrieval, as evidenced by the performance metrics in Table~\ref{tab:mbeir}, {\em i.e.}, directly employing Qwen2-VL-7B~\cite{wang2024qwen2} for retrieval tasks results in inferior performance. To address this issue, we start by adapting LMMs for text-to-text retrieval by training LoRA modules on the Natural Language Inference (NLI) dataset~\cite{gao2021simcse}, consisting pairs of text samples that are ideal to enhance LMMs for retrieval. For further discussion on the selection of pre-training datasets, please refer to the supplementary material. 

\vspace{2pt}
\noindent \textbf{Stage-II: Instruction Tuning for Universal Retrieval.} 
To further enhance the retrieval capabilities of the LMMs across various multimodal retrieval tasks, we train on M-BEIR, which comprises 8 distinct retrieval tasks with 10 different datasets, as curated by~\cite{wei2023uniir}, 
%Unlike the pre-training stage, the instruction-tuning here extends training across eight different tasks, 
including image-to-image retrieval, composed image retrieval, and image/question-to-multimodal-document retrieval, among others. 
For different retrieval tasks, we incorporate task-specific instructions tailored for each retrieval type. For example, to complete an image-to-image retrieval task, the instruction can be ``\textit{retrieval a similar image.}" For further details regarding the instructions and M-BEIR datasets, please refer to the supplementary material.

\vspace{2pt}
\noindent \textbf{Training Objective.} 
We employ contrastive learning with the InfoNCE loss~\cite{oord2018representation} for both language-only pre-training and instruction tuning stages. 
Specifically, given a batch size of $B$, the embeddings of $n$-th query $q_n$ should be positioned close to the embeddings of its positive target $c_n$ and far away from other negative instances, formulated as: 
\begin{equation*}
\mathcal{L}_{\text{ret}}=-\frac{1}{B} \sum_{n=1}^B \log \left[\frac{\exp \left[ \kappa\left(\texttt{LMM}(q_n), \texttt{LMM}(c_n)\right) / \tau \right]}{\sum_{m=1}^B \exp \left[ \kappa\left(\texttt{LMM}(q_n), \texttt{LMM}(c_m)\right) / \tau \right]}\right]
\end{equation*}
% \weidi{the introduced notation has never been used here, for example, $\Phi_{\text{ret}}$ introduced in Sec.~3.1. or change your notations in the formulation accordingly.}

\noindent where $\tau$ refers to the temperature parameter, and $\kappa(\cdot,\cdot)$ denotes the cosine similarity. Additionally, $\texttt{LMM}(\cdot)$ represents the feature extraction process with LMMs, as mentioned in Section~\ref{sec:feature_extraction}. 
The model after both pre-training and instruction tuning is referred as \textbf{LamRA-Ret}.

% \weidi{I would suggest to add a paragraph on `Training'. 
% Unify the Stage-I, and Stage-II into one training scheme.}

\subsection{Training for Reranking}
\label{sec:reranking}

Here, we exploit the flexibility of LMMs to process multiple images or long texts and train a lightweight LoRA module to adapt them for reranking. 
As a result, we propose \textbf{LamRA-Rank}, 
which supports inputs of single or multiple candidates from the outputs of LamRA-Ret, to further improve the retrieval performance.

\vspace{2pt}
\noindent \textbf{Collecting Training Data for Reranking.} 
Here, we employ the LamRA-Ret model trained in Section~\ref{sec:training_for_retrieval} as the initial retriever, and train the reranking model on its top 100 retrieved candidates and use them as hard negatives. This approach enables LamRA-Rank to acquire a more nuanced understanding and improve its ranking performance.

\vspace{2pt}
\noindent \textbf{Joint Training for Pointwise and Listwise Reranking.} 
Given that the LMMs can accept flexible inputs, we explore joint training for both pointwise and listwise reranking.

In the case of pointwise reranking, for any query ($q$), 
we randomly select a negative candidate ($c_{\text{neg}}$) from the top 100 candidates and instruct the LamRA-Rank to output \texttt{YES} for the ground truth ($c_{\text{pos}}$) and \texttt{NO} for the negative candidate. Cross-entropy loss is employed as the loss function, expressed as $\mathcal{L}_{\text{point}} = \mathcal{L}_{\text{ce}}(\texttt{YES}, \texttt{Reranker}(q, c_{\text{pos}})) + \mathcal{L}_{\text{ce}}(\texttt{NO}, \texttt{Reranker}(q, c_{\text{neg}})),$ where $\texttt{Reranker}(\cdot,\cdot)$ represents the autoregressive output process of LamRA-Rank.
% \weidi{don't understand the notations $q$, $t$, $\texttt{Reranker}$ they have never been explained.}

In contrast, for listwise reranking, we randomly select $M$ negative samples $(c_1, c_2, \cdots, c_M)$ from the top 100 candidates, where $M$ is a randomly determined integer between 2 and 5. We then randomly insert the ground truth $(c_{\text{pos}})$ at any position and prompt the LamRA-Rank to directly output the position number of the ground truth. This process can be formulated as $\mathcal{L}_{\text{list}} = \mathcal{L}_{\text{ce}}(\texttt{GT-POSITION}, \texttt{Reranker}(q, c_{\text{pos}}, c_1, c_2, \cdots, c_M)).$

% \weidi{same problem as Sec.~3.3, you need to use your introduced notation, for example, $\Phi_{\text{rerank}}$ introduced in Sec.~3.1. or change your notations in the formulation accordingly.}

% \weidi{Same problem as before, there should be a place to formally introduce reranking with LMMs.}

The final loss is a weighted sum: $\mathcal{L}_{\text{rank}} = \mathcal{L}_{\text{point}} + \mathcal{L}_{\text{list}}$. 

\subsection{Inference Pipeline}
\label{sec:inference}

\noindent At the inference stage, we employ LamRA-Ret for the initial retrieval phase~($\Phi_{\text{ret}}$) and LamRA-Rank for the subsequent reranking~($\Phi_{\text{rank}}$). 
Given a query ($q$) and a candidate set ($\Omega$), LamRA-Ret is first utilized to compute an embedding similarity score ($S_{\text{ret}}$) for each candidate based on cosine similarity. Subsequently, the candidates are sorted to obtain the top-$K$ candidate set ($\mathcal{C}_1$). For the reranking process, we offer two options: pointwise reranking and listwise reranking. In the case of pointwise reranking,  the query and each of the top-$K$ candidates are sequentially input into the LMM, performing $K$ inference operations and assigning a reranking score ($S_{\text{rank}}$) to each candidate. This reranking score comes from the probability of the LMMs outputting \texttt{YES} for each candidate. Conversely, for listwise reranking, the query and the top-$K$ candidates are simultaneously fed into LamRA-Rank, which directly output the serial number of the most relevant candidate. More discussion on these two methods can be found in Section~\ref{sec:ablate}. In the final step, the embedding similarity score from LamRA-Ret and the reranking score from LamRA-Rank are aggregated into a weighted sum to get the final score: $S = \alpha \times S_{\text{ret}} + (1 - \alpha) \times S_{\text{rank}}$, where $\alpha$ is a weight hyperparameter. This final score is then used to generate the reordered candidate set ($\mathcal{C}_2$). We refer to the combined framework of LamRA-Ret and LamRA-Rank as \textbf{LamRA}.
\vspace{2pt}


% \weidi{The scores, $S_{\text{ret}}$, $S_{\text{rank}}$ have not been linked to previous equations, how are they acquired.}

% \jc{Maybe we can add a subsection here to compare and discuss the existing works like UniIR to make the reviewer better understand your contribution. After going through the previous sections, it seems you have not systematically talk about this. }

% \begin{equation}
% \small
% \mathcal{L}_{\text{point}} = - \log p(\text{No} \mid \text{Prompt}_{\text{point}}, q, c) - \log p(\text{Yes} \mid \text{Prompt}_{\text{point}}, q, t)
% \end{equation}

% \begin{equation}
% \small
% \mathcal{L}_{\text{list}} = - \sum_{t=1}^{T} \log p(a^t \mid \text{Prompt}_{\text{list}}, q, t, c_1, ..., c_m, a^{1:t-1})
% \end{equation}




% \weidi{the sentence has been mentioned several times, but never explained what does it mean.}
% As mentioned in Section~\ref{sec:feature_extraction}, the features extracted by the LMM from different modalities are mapped into the same feature space, specifically the hidden space of the LLM. This shared feature space links image and text features, enabling improvements in both even when training with data from only one modality. This means that training with pure text or pure image data can simultaneously enhance the model's ability to extract features from both modalities. We ultimately choose to conduct training on the Natural Language Inference (NLI) dataset~\cite{gao2021simcse}, further discussion on the pre-training datasets is provided in the Appendix.
% \weidi{this section needs to be rewritten, 
% there is no need to explain shared space of image and text, or training one can enhance the model's ability from both modalties. Simply say, we start by tuning LLMs for text-to-text retrieval, as it has originally trained with generative tasks only, blabla...}

% \weidi{explain how this is trained, refer to the formulation in Sec.~3.1, for example, no image is provided ? }


==> section/03-method_old.tex <==
\section{Method}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{pics/architecture_print.pdf} \\
  \vspace{-6pt}
  \caption{\textbf{Overview of the proposed LamRA framework.} LamRA consists of two components: LamRA-Ret and LamRA-Rank. The top section illustrates LamRA-Ret, encompassing both the pre-training and instruction-tuning stages, where contrastive learning is employed to enhance the retrieval capability of LMMs. The pre-training stage aims to improve the feature extraction capabilities through text-to-text retrieval, while the instruction tuning stage adapts the LMMs to various retrieval tasks by fine-tuning on diverse tasks with task-specific instructions. The bottom section depicts the joint training process of LamRA-Rank, which integrates both pointwise and listwise reranking.
  \weidi{this figure seems to take too much vertical space, try to shrink a bit.}}
    \vspace{-4pt}
 \label{fig:arch}
\end{figure*}


\noindent This section starts by formulating our considered problem in Section~\ref{sec:problem_formulation}; then we elaborate on the architecture and feature extraction process in Section~\ref{sec:feature_extraction}; and describe the training details to equip the LMMs with retrieval capability in Section~\ref{sec:training_for_retrieval}; lastly, we present the approach to endow the LMMs with universal reranking abilities, aiming to further boost retrieval performance, as discussed in Section~\ref{sec:reranking}. 

\subsection{Problem Formulation} 
\label{sec:problem_formulation}

\noindent We address the challenge of universal retrieval and reranking with a generative model. Specifically, for one specific query~($q$), which can be an image, text, or an interleaved image-text format, and a retrieval set of $N$ candidates $\Omega = \{c_1, c_2, \cdots, c_N\}$ where each $c_i$ comprises images, text, or interleaved formats, we first extract the embeddings for both the query and all candidates with LMMs, and rank all candidates in $\Omega$ based on the relevance, 
{\em i.e.}, cosine similarity between the query and candidate embeddings. 
This initial retrieval process yields the top-$K$ candidates, represented as $\mathcal{S}_1 = \Phi_{\text{ret}}(q, \Omega)$. Subsequently, we refine this subset through a reranking process to produce the final ranked output, denoted as $\mathcal{S}_2 = \Phi_{\text{rerank}}(q, \mathcal{S}_1)$. Here, $\mathcal{S}_2$ represents the final reordered set of candidates.

In the following section, we provide details on extracting features for queries and candidates of arbitrary format.

% \weidi{need to provide more details, 
% how images and texts are encoded, and get the embedding, 
% then what is the task, i.e., rank the cases in a pool by relevance score, .... 
% what does reranking looks like,....}
% \weidi{need to provide a formulation for this universal retrieval problem, for example, assume a set of images $\mathcal{I} = \{I_1, I_2, \dots, I_n\}$, ...}

\subsection{Architecture \& Feature Extraction}
\label{sec:feature_extraction}

\noindent The architecture of LMMs typically consists of three main components: a vision encoder, a vision projector, and a language model.
To compute the embedding with a generative model, 
we adopt a similar approach as ~\cite{jia2021scaling, jiang2024e5},
using an Explicit One-word Limitation (EOL). 
Specifically, we adopt the following prompts: 
(i) for image-only input, we use \texttt{<image> Summarize the above image in one word: <emb>}, where \texttt{<image>} is a placeholder for the input image. 
(ii) for text-only input, we use: \texttt{<text> Summarize the above sentence in one word: <emb>}, where $\texttt{<text>}$ is a placeholder for the input sentence. (iii) for mixed image-text input, we use the prompt: \texttt{<image\textsubscript{1}><text\textsubscript{1}>...<image\textsubscript{i}><text\textsubscript{j}> Summarize the above image and sentence in one word: <emb>.} For any combination of images and text inputs, the LMM uses the vision encoder and vision projector to map images into language space, which are then processed alongside the text by the large language model. After processing, we select the last hidden state of the position immediately preceding the \texttt{<emb>} token as the representation of the input.

\subsection{Training for Retrieval} 
\label{sec:training_for_retrieval}

\vspace{3pt}\noindent 
In this section, we describe a two-stage training scheme, to advance the retrieval capabilities of LMMs. The first stage involves language-only pre-training, which facilitates the generative model to output improved embeddings. 
The second stage, instruction tuning, further adapts the LMMs to a wide range of retrieval tasks.

% In this section, we describe a two-stage training scheme, to advance the retrieval capabilities of LMMs. 
% The first stage involves language-only pre-training, concentrating on strengthening the LMMs' capability to extract features in response to summarization prompts. The second stage, instruction tuning, further enhances the model’s adaptability to various retrieval tasks.

 %To progressively enhance the retrieval capabilities of the LMMs, we first improve the model's capability to extract features in response to summarization prompts. Since LMMs are originally trained solely for generative tasks, their capability to extract features in response to summarization prompts is relatively limited, as shown in Table~\ref{tab:mbeir}. Therefore, we begin by tuning LMMs for text-to-text retrieval to improve their feature extraction ability. Specifically, we conduct training on the Natural Language Inference (NLI) dataset~\cite{gao2021simcse}, which consists of paired text samples. 
 
\vspace{3pt}
\noindent \textbf{Stage-I: Adapting LMMs for Retrieval Tasks.} LMMs were predominantly trained for generative tasks, {\em e.g.}, next-token prediction, which limits their ability for retrieval, as evidenced by the performance metrics in Table~\ref{tab:mbeir}. 
To address this issue, we start by adapting LMMs for text-to-text retrieval by training LoRA modules on the Natural Language Inference (NLI) dataset~\cite{gao2021simcse}, consisting pairs of text samples that are ideal to enhance LMMs for retrieval. 

We employ contrastive learning with  InfoNCE loss~\cite{oord2018representation}, given a batch size of $B$, the embeddings of $n$-th query text $q_n^t$ should be positioned close to the embeddings of its positive target text $c_n^{t}$ and far away from other negative instances, which can be formulated as:
\begin{equation*}
\mathcal{L}_{\text{ret}}=-\frac{1}{B} \sum_{n=1}^B \log \left[\frac{\exp \left[ \kappa\left(\texttt{LMM}(q_n^t), \texttt{LMM}(c_n^t)\right) / \tau \right]}{\sum_{m=1}^B \exp \left[ \kappa\left(\texttt{LMM}(q_n^t), \texttt{LMM}(c_m^t)\right) / \tau \right]}\right]
\end{equation*}
\weidi{the introduced notation has never been used here, for example, $\Phi_{\text{ret}}$ introduced in Sec.~3.1. or change your notations in the formulation accordingly.}

\noindent where $\tau$ refers to the temperature parameter, and $\kappa(\cdot,\cdot)$ denotes the cosine similarity. Additionally, $\texttt{LMM}(\cdot)$ represents the feature extraction process with LMMs, as mentioned in Section~\ref{sec:feature_extraction}.
For further discussion on the selection of pre-training datasets, 
please refer to the supplementary materials.

\vspace{3pt}
\noindent \textbf{Stage-II: Instruction Tuning for Universal Retrieval.} 
To further enhance the retrieval capabilities of the LMMs across various multimodal retrieval tasks, we train on M-BEIR, that comprises 8 distinct retrieval tasks with 10 different datasets, as curated by~\cite{wei2023uniir}.
%making it a valuable instructional training dataset for our purposes.

Unlike the language-only stage, the instruction-tuning here extends training across eight different tasks, including image-to-image retrieval, composed image retrieval, and image/question-to-multimodal-document retrieval, among others. To better adapt LMMs to these diverse retrieval tasks, we incorporate task-specific instructions tailored for each retrieval type. 
The training process during the instruction-tuning stage also employs contrastive learning, where each query consists of an instruction paired with the corresponding image, text, or image-text input, 
while candidates span various types as well. 
For further details regarding the instructions and M-BEIR datasets, please refer to the supplementary materials. We refer to the model after completing both the pre-training and instruction tuning stages as \textbf{LamRA-Ret}.

\weidi{I would suggest to add a paragraph on `Training'. 
Unify the Stage-I, and Stage-II into one training scheme.}

\subsection{Training for Reranking}
\label{sec:reranking}

Here, we exploit the flexibility of LMMs to process multiple images or long texts and train a lightweight LoRA module to adapt them for reranking. 
As a result, we propose \textbf{LamRA-Rank}, which supports inputs of single or multiple candidates from the outputs of LamRA-Ret, to further improve retrieval performance.

\vspace{3pt}
\noindent \textbf{Collecting Training Data for Reranking.} 
In order to train the reranking model, we employ the LamRA-Ret model trained in Section~\ref{sec:training_for_retrieval} as the initial retriever. Specifically, for each query in M-BEIR, we retain the top 100 results retrieved by LamRA-Ret and use these as hard negatives for training LamRA-Rank. This approach enables LamRA-Rank to acquire a more nuanced understanding and improve its ranking performance.

\vspace{3pt}
\noindent \textbf{Joint Training for Pointwise and Listwise Reranking.} Given that the LMMs can accept flexible inputs, we explore joint training for both pointwise and listwise reranking.

In the case of pointwise reranking, for any query \kun{($q$)}, 
we randomly select a negative candidate \kun{($c_{\text{neg}}$)} from the top 100 candidates and instruct the LamRA-Rank to output \texttt{YES} for the ground truth \kun{($c_{\text{pos}}$)} and \texttt{NO} for the negative candidate. Cross-entropy loss is employed as the loss function, expressed as \kun{$\mathcal{L}_{\text{point}} = \mathcal{L}_{\text{ce}}(\texttt{YES}, \texttt{Reranker}(q, c_{\text{pos}})) + \mathcal{L}_{\text{ce}}(\texttt{NO}, \texttt{Reranker}(q, c_{\text{neg}})),$} where $\texttt{Reranker}(\cdot,\cdot)$ represents the autoregressive output process of LamRA-Rank.
% \weidi{don't understand the notations $q$, $t$, $\texttt{Reranker}$ they have never been explained.}

In contrast, for listwise reranking, we randomly select $M$ negative samples \kun{$(c_1, c_2, \cdots, c_M)$} from the top 100 candidates, where $M$ is a randomly determined integer between 2 and 5. We then randomly insert the ground truth \kun{$(c_{\text{pos}})$} at any position and prompt the LamRA-Rank to directly output the position number of the ground truth. This process can be formulated as \kun{$\mathcal{L}_{\text{list}} = \mathcal{L}_{\text{ce}}(\texttt{GT-POSITION}, \texttt{Reranker}(q, c_{\text{pos}}, c_1, c_2, \cdots, c_M)).$}

\weidi{same problem as Sec.~3.3, you need to use your introduced notation, for example, $\Phi_{\text{rerank}}$ introduced in Sec.~3.1. or change your notations in the formulation accordingly.}

% \weidi{Same problem as before, there should be a place to formally introduce reranking with LMMs.}

The final loss is a weighted sum: $\mathcal{L}_{\text{rank}} = \mathcal{L}_{\text{point}} + \mathcal{L}_{\text{list}}$. Incorporating the pointwise and listwise reranking provides two options for the inference stage. For pointwise reranking, we sequentially input the query and each of the top-$K$ candidates into the LMM, performing $K$ inference operations and assigning a reranking score to each candidate. This reranking score represents the probability of the LMMs outputting \texttt{YES} for each candidate. In contrast, for listwise reranking, we simultaneously feed the query and the top-$K$ candidates into the LamRA-Rank and directly output the serial number of the most relevant candidate. More discussion on these two methods can be found in Section~\ref{sec:ablate}. In the final step, we aggregate the feature similarity score ($S_{\text{ret}}$) from the LamRA-Ret and the reranking score ($S_{\text{rank}}$) from LamRA-Rank into a weighted sum to get the final score: $S = \alpha \times S_{\text{ret}} + (1 - \alpha) \times S_{\text{rank}}$, where $\alpha$ is a weight hyperparameter. We refer to the combined framework of LamRA-Ret and LamRA-Rank as \textbf{LamRA}.
\weidi{The scores, $S_{\text{ret}}$, $S_{\text{rank}}$ have not been linked to previous equations, how are they acquired.}

% \jc{Maybe we can add a subsection here to compare and discuss the existing works like UniIR to make the reviewer better understand your contribution. After going through the previous sections, it seems you have not systematically talk about this. }

% \begin{equation}
% \small
% \mathcal{L}_{\text{point}} = - \log p(\text{No} \mid \text{Prompt}_{\text{point}}, q, c) - \log p(\text{Yes} \mid \text{Prompt}_{\text{point}}, q, t)
% \end{equation}

% \begin{equation}
% \small
% \mathcal{L}_{\text{list}} = - \sum_{t=1}^{T} \log p(a^t \mid \text{Prompt}_{\text{list}}, q, t, c_1, ..., c_m, a^{1:t-1})
% \end{equation}




% \weidi{the sentence has been mentioned several times, but never explained what does it mean.}
% As mentioned in Section~\ref{sec:feature_extraction}, the features extracted by the LMM from different modalities are mapped into the same feature space, specifically the hidden space of the LLM. This shared feature space links image and text features, enabling improvements in both even when training with data from only one modality. This means that training with pure text or pure image data can simultaneously enhance the model's ability to extract features from both modalities. We ultimately choose to conduct training on the Natural Language Inference (NLI) dataset~\cite{gao2021simcse}, further discussion on the pre-training datasets is provided in the Appendix.
% \weidi{this section needs to be rewritten, 
% there is no need to explain shared space of image and text, or training one can enhance the model's ability from both modalties. Simply say, we start by tuning LLMs for text-to-text retrieval, as it has originally trained with generative tasks only, blabla...}

% \weidi{explain how this is trained, refer to the formulation in Sec.~3.1, for example, no image is provided ? }


==> tables/ablate.tex <==
\begin{minipage}[t]{0.2\textwidth} % [t] 对齐顶部
    \centering
    \scriptsize
    % Table 10
    \begin{adjustbox}{valign=t} % 垂直对齐顶部
    \begin{tabular}{ccc}
    \toprule
    Pre. & Inst. & \textbf{Avg.} \\
    \midrule
    \ding{56} & \ding{56} & 23.0\\
     \ding{52} & \ding{56} & 36.2\\
     \ding{56} & \ding{52} & 53.6\\
     \ding{52} & \ding{52} & 56.6\\
    \bottomrule
  \end{tabular}
    \end{adjustbox}
    \captionof{table}{\textbf{Effect of the two-stage training.}}
\end{minipage}%
\begin{minipage}[t]{0.2\textwidth} % [t] 对齐顶部
    \centering
    \scriptsize
    % Table 11
    \begin{adjustbox}{valign=t} % 垂直对齐顶部
    \begin{tabular}{cccc}
    \toprule
    \textbf{LMM} & \textbf{Ret} & \textbf{Rank} & \textbf{Avg.} \\
    \midrule
     \multirow{2}{*}{Qwen2-VL-2B} & \ding{52} & \ding{56} & 51.6\\
      & \ding{52} & \ding{52} & x\\
      \midrule
     \multirow{2}{*}{Qwen2-VL-7B} & \ding{52} & \ding{56} & 56.6\\
      & \ding{52} & \ding{52} & 63.7\\
    \bottomrule
  \end{tabular}
    \end{adjustbox}
    \captionof{table}{Table 11}
\end{minipage}
